Automatic Controllable Colorization via Imagination

We propose a framework for automatic colorization that allows for iterative editing and modifications. The core of our framework lies in an imagination module: by understanding the content within a grayscale image, we utilize a pre-trained image generation model to generate multiple images that contain the same content. These images serve as references for coloring, mimicking the process of human experts. As the synthesized images can be imperfect or different from the original grayscale image, we propose a Reference Refinement Module to select the optimal reference composition. Unlike most previous end-to-end automatic colorization algorithms, our framework allows for iterative and localized modifications of the colorization results because we explicitly model the coloring samples. Extensive experiments demonstrate the superiority of our framework over existing automatic colorization algorithms in editability and flexibility. Project page: https://xy-cong.github.io/imagine-colorization.

==> 03_preliminary.tex <==
% \section{Preliminary}
% \label{sec:Preliminary}



==> figs/templete.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    % \includegraphics[width=\linewidth]{}
    \caption{Caption.}
    \label{fig:template}
\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/templete.tex <==
\begin{table}[t]
\centering
% \resizebox{\columnwidth}{!}{%

\begin{tabular}{lc}
\toprule
Method & Accuracy \\
\midrule
Ours & 0.502 \\
\bottomrule
\end{tabular}

% }
\caption{
Caption goes here
}
\vspace{-0.05in}
\label{tab:template}
\end{table}

